A Comprehensive Study on Artificial Intelligence Algorithms to Implement Safety Using Communication Technologies

The recent development of artificial intelligence (AI) has increased the interest of researchers and practitioners towards applying its techniques into multiple domains like automotive, health care and air space to achieve automation. Combined to these applications, the attempt to use AI techniques into carrying out safety issues is momentarily at a progressive state. As AI problems are getting even more complex, large processing power is demanded for safety-critical systems to fulfill real-time requirements. These challenges can be solved through edge or cloud computing, which makes the communication an integral part of the solution. This study aims at providing a comprehensive picture of the state of the art AI based safety solutions that uses different communication technologies in diverse application domains. To achieve this, a systematic mapping study is conducted and 565 relevant papers are shortlisted through a multistage selection process, which are then analyzed according to a systematically defined classification framework. The results of the study are based on these main objectives: to clarify current research gaps in the field, to identify the possibility of increased usage of cellular communication in multiple domains, to identify the mostly used AI algorithms and to summarize the emerging future research trends on the topic. The results demonstrate that automotive domain is the one applying AI and communication the most to implement safety and the most used AI in this domain is neural networks, clustering and computer vision; applying cellular communication to automotive domain is highest; the use of non-cellular communication technologies is dominant however a clear trend of a rapid increase in the use of cellular communication is observed specially from 2020 with the roll-out of 5G technology.

==> 1st submission backup/classification.tex <==
\section{Classification Scheme} 
\label{sec:classscheme}

This section presents the classification schemes developed in this study to address the research questions. 

\subsection{AI algorithm classification}
% Based on the initial categorization %\sara{here we need to explain to the readers what do we mean by initial categorization } 
% and the later \textit{keywording}, %\sara{\textit{keywording}},
% the classification was shaped as follows. For each {data item} of this facet a short description is presented .  
% \textcolor{red}{Link to appendix B}
Classes were obtained from an initial categorization and \textit{keywording} (see Appendix~\ref{sec:appendix_B}). For each {data item} of this facet a short description is presented as follows:

%\renewcommand\labelitemi{\textendash}
\begin{itemize}
    \item \textcolor{blue}{\textit{Clustering} - An unsupervised learning method that groups similar data without having the target features in the training data \cite{xu2008clustering}. Outputs might be less accurate compared to supervised methods due to the absence of expert knowledge input during the training. Examples of methods are K-means, DBSCAN and MeanShift.}
    \item \textit{Cognitive Architecture} - Aims to use the research of cognitive psychology in order to create artificial computational system processes reasoning like humans \cite{lieto2018role}. Although complex behaviors can be modeled, the development of such architectures might require some effort. Soar, COGNET and CLARION are examples of cognitive architectures.
    \item \textit{Computer Vision} - It is a class of problem that relates to the process of automating the visual perception by including tasks from low-level vision as noise removal or edge sharpening to high-level vision by segmenting the images or interpreting the scene \cite{bezdek1999image}.
    This class includes primary studies in the field of image processing, virtual reality, or augmented reality.
    
    \textcolor{red}{Good to mention that this is not exactly AI algorithm but it can be implemented using AI algorithm and thats why we think that it is importnt to keep this here.}
    \item \textit{Fuzzy logic system} - Solves a problem through a set of If-Then rules that takes into account the uncertainties in the inputs and outputs by imitating human decision-making \cite{dadios2012fuzzy}. As these rules are written in natural language, this method provides explainability of the decisions. However, it demands a manual process to model the rules and the models might have lower accuracy as compared to other AI algorithms.
    \item \textit{Natural Language Processing (NLP)} - It is a class of problem that studies mechanisms to make the computer program understand the human language.
    % Aims at improving the ability of a computer program in understanding the human language. 
    \item \textit{Neural Network (NN)} - Refers to a set of algorithms designed to simulate the connection between the neurons \cite{ripley2007pattern}. This method has large popularity given the ability to solve complex problems in different fields. As a drawback, it demands NN architectures with thousands or millions of neurons, which makes necessary large dataset to train the model and lead to high inference times. Examples of NN include multilayer perceptron (MLP), Long short-term memory (LSTM) and Deep Neural Network (DNN).
    \item \textit{Ontology} - Refers to a formal and structural way of representing concepts, relations or attributes in a domain \cite{fensel2001ontologies}. This requires a domain expert knowledge to design the ontology and the usage of a specific language.
    \item \textit{Optimization} - Class of an iterative procedures that aims at achieving ideally the optimal solution of a problem beginning from a guessed solution \cite{ruder2016overview}.  
    \item \textit{Regression Analysis} - Studies the relationship between a dependent and independent variable to models a function that makes predictions. The model is obtained by iteratively adjusting the function parameters to map a given set of input and outputs \cite{bishop2006pattern}. Usually it is applied to problems that are linearly separable.
    \item \textit{Reinforcement Learning (RL)} - Class of methods that determines optimal actions that maximizes the reward of an agent that is continuously exploring the state space and taking observations \cite{Sutton2018}. It is widely applied in problems that involves automating the decision taken by an intelligent agent. Q-learning and its DNN variant, DQN, are examples of RL methods.
    \item \textit{Finite State Machine (FSM)} - Represents a computational model that performs predefined actions depending on a series of events \cite{gladyshev2004finite}. It requires knowledge from the domain expert to model the states and the transitions between them. Commonly, it is used in tasks that involves simple decisions. Hierarchical FSM and fuzzy state machine are examples of FSM algorithms.
    \item \textit{Non-specified} - Relates to primary studies that mention the use of AI or ML, but do not elaborate into a particular technique.   
    \item \textit{Other} - Relates to primary studies that use a AI technique that is not part of the above-mentioned ones. 
\end{itemize}


\subsection{Communication technology classification}
\label{sec:comm_tec_class}
% \textcolor{red}{Link to appendix B}
Based on the initial categorization for communication and the process of keywording, the following classes were extracted (see Appendix~\ref{sec:appendix_B}): 
% \textcolor{red}{do we need references in this section ? Maybe a ref of a book on communication technologies}

\begin{multicols}{2}
    \begin{itemize}
        \item \textit{Cellular  
        \item Non-cellular 
       % \item Satellite
        \item Not-mentioned}
    \end{itemize}
\end{multicols}

To address the first and second research questions (RQ1, RQ2), cellular and non-cellular communication technologies are further divided into subcategories. This is necessary to investigate which of the communication technologies are mostly used to implement safety in different application domains and which of the non-cellular communication technologies can be potentially replaced with the cellular ones \cite{Naik2020}: 

\subsubsection{Cellular communication technology classification}

\begin{itemize}
    \item \textit{2G} - Second generation of cellular communication technology that incorporated digital speech and medium-rate data transfer. GSM, GPRS and EDGE are also other terms used for 2G.
    \item \textit{3G} - The third generation brought higher speed data transfer and improved quality in the services compared to 2G. WCDMA is also referred to 3G technology.
    \item \textit{4G} - A higher data transfer rate leveraged new use-cases such as IoT and industry automation. LTE is another term usually associated to 4G.
    \item \textit{5G} - Low latency communication with high data rate made possible to expand the use-cases to diverse domains.
    \item \textit{Cellular (not-specified)}: Category used to group studies that do not mention which cellular technology used in the T-A-K fields.
\end{itemize}


\subsubsection{Non-Cellular communication technology classification}

\begin{itemize}
    \item \textit{WiFi} - Includes communication technologies based on IEEE 802.11 standard, such as vehicular ad hoc networks (VANET) and dedicated short range communication (DSRC).
    \item \textit{Radio-frequency identification (RFID)}: A short distance communication technology that uses electromagnetic field to transfer data.
    \item \textit{Bluetooth} - Communication technology intended for low energy consumption, short range communication and low data transfer rate.
    \item \textit{Satellite} - Long range communication technology, however sensitive to noises and dependent on line of sight.  
    \item \textit{Non-cellular (not-specified)} - Comprises studies that do not specify the employed non-cellular technology in the T-A-K fields. 
\end{itemize}


\subsection{Application domain classification}
\label{sec:application_domain}

From keywording, the following classification scheme was derived for the domains where safety is provided by applying AI:

%\begin{multicols}{2}
    \begin{itemize}
        % \item \textit{Agriculture} - Covers agricultural automation for cropping fields.
        \item \textit{Air space} - Includes unmanned aerial vehicles (UAV) and airport management systems.
        % \textcolor{red}{we need to explain three of them. others are self-explanatory}
        \item \textit{Automotive} - Encompasses intelligent transportation systems, with predominance of advanced driver-assistance systems (ADAS), autonomous vehicles and truck platooning.
        \item \textit{Construction} - Monitoring of building infrastructure and monitoring of construction workers.
        \item \textit{Education} - Includes personal training and academic learning applications.
        \item \textit{Factory} - Mainly covers warehouses, chemical industries and nuclear plants.
        \item \textit{Health care} - Referees to automation of patient care and remote surgeries.
        \item \textit{Marine} - Underwater applications and unmanned surface vehicles (USVs).
        \item \textit{Mining} - Covers monitoring of mining workers and autonomous underground machinery.
        \item \textit{Robotics} - Comprises utilization of robots for process automation.
        \item \textit{Surveillance} - Environment monitoring for security.
        \item \textit{Telecommunication} - Applications in the communication domain, such as enhancements in the reliability and traffic capacity.
        \item \textit{Other} - Specifies studies that do not fit in the aforementioned application domains. 
    \end{itemize}
%\end{multicols}


\subsection{Research contribution classification}
\label{sec:research_contribution}

By defining a classification framework for \textit{types of research contribution}, new methods, techniques or tools can be developed in the future by the researchers to implement safety. In order to categorize this facet, the classification scheme presented and defined by Petersen et al. in \cite{petersen2008systematic} is used. This scheme is highly adopted by researchers when conducting a systematic mapping study~\cite{asadollah201710}. This facet was formed with the following \textit{data items}:

% \renewcommand\labelitemi{\textbullet}
\begin{itemize}
  \item  \textit{Model} - Refers to studies that present information and abstractions to be used in AI-based safety.    
  \item  \textit{Method} - Refers to general concepts and detailed working procedures that address specific concerns about implementing AI-based safety.  
  \item  \textit{Metric} - Refers to specific  measurements and metrics to assess certain properties of AI-based safety.
  \item  \textit{Tool} - Refers to any kind of tool or prototype that can be employed in the current models.
  \item  \textit{Open Item} - Refers to the remaining studies that do not belong to any of the above mentioned categories.
\end{itemize}


\subsection{Research types classification}
\label{sec:research_type}

% According to \cite{asadollah201710}, the \textit{research types} classification is chosen, because of the importance on understanding the research approach and the value it represents. 
To categorize the \textit{research types}, the classification scheme proposed by Wieringa et al. in \cite{wieringa2006requirements} was applied, which includes the following \textit{data items}: 

\begin{itemize}
  \item  \textit{Validation Research} - Investigates the novel techniques, that are yet to be implemented in the practice. Examples of investigations include experiments, prototyping and simulations.
  \item  \textit{Evaluation Research} - Evaluates an implemented solution in practice considering the benefits and drawbacks of this solution. It includes case studies, field experiments and related studies.    
  \item  \textit{Solution Proposal} - Refers to a novel solution for a problem or a significant extension to an existing one.
  \item  \textit{Conceptual Proposal} - Gives a new approach at looking topics by structuring them in conceptual frameworks or taxonomy.
  \item  \textit{Experience Paper} - Reflects the experience of an author explaining at what extent something is performed in practice.  
  \item  \textit{Opinion Paper} - Refers to studies that mostly express the opinion of the authors on certain methods.  
\end{itemize}



==> 1st submission backup/method.tex <==
\section{Study Method} 
\label{sec:study_method}

The systematic mapping (SM) method is employed in this study to understand how the field of AI-based safety enabled by communication technology is evolving. Essentially, SM performs an overview of research works to answer key research questions of this field. The SM analysis is also supported by visual maps that bring temporal and quantitative perspectives of different aspects of the study field. The SM process can be performed in different manners. 
In this study we follow the guidelines from \cite{kitchenham2007guidelines, wohlin2012experimentation}  and divide the overall process into three main classical phases for systematic mapping studies: planning, conducting, and documenting, and then further divide each phase into multiple steps as depicted in Figure \ref{fig:process} and described below.
%[8] B. A. Kitchenham, S. Charters, Guidelines for performing systematic literature reviews in software engineering, Tech. Rep. EBSE-2007-01, Keele University and University of Durham (2007).
%[9] C. Wohlin, P. Runeson, M. H¨ost, M. Ohlsson, B. Regnell, A. Wessl´en, Experimentation in Software Engineering, Computer Science, Springer, 2012.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{sms_studyProcess.PNG}
    \caption{Overview of the research method process and its main activities.}
    \label{fig:process}
\end{figure}

%In this study we adopted the guidelines from [REF], which is comprised by five steps: Definition of research questions; Search string and source selection; Definition of study selection criteria; Data extraction; and data analysis. Each of these steps are detailed in the next sections.
\textbf{Planning: } The first phase in the study process and it aims at (i) demonstrating the need for performing a mapping study on the use of AI algorithms using communication in diverse domains to implement safety;
%on safety for MRSs; indeed, as discussed also in Section 9, secondary studies exist on topics related to robotics safety like mechanical and controller design [20] and human-robot interaction [21, 22, 23], but none of them takes into consideration safety from a software engineering point of view; 
(ii) defining the main research questions (see Section \ref{sec:rqs}); and (iii) defining the search string and selecting the scientific online digital libraries to perform the systematic mapping study (see Section \ref{sec:stringSource}).

\textbf{Conducting: } This phase consists of the following steps: 

\begin{enumerate}[label=(\roman*)]
\item \textit{Study retrieval}: The final search string is applied to the short-listed well-known academic search databases (see Section \ref{sec:studyretrieval}). The output of this activity is a comprehensive list of all candidate studies resulting from the search in the digital libraries.

\item \textit{Study selection}: Duplicates are removed from the candidate entries. Then entries are filtered first using the inclusion and exclusion criteria, and second using the Title-Abstract-Keywords (T-A-K) criteria (see Section \ref{sec:studySelection}) to obtain the final list of relevant studies to be considered in later steps of the study.

\item \textit{Classification scheme definition}: The next step in the systematic mapping study is to establish how the relevant studies are going to be classified. The classification scheme are designed to collect data for addressing the research questions \cite{wohlin2012experimentation} as formulated in the planning phase. The process of defining the classification scheme is described in Section~\ref{sec:classification}, and the obtained classifications are explained in Section~\ref{sec:classscheme}. %including the clusters for keywording method.

\item \textit{Data extraction}: Each selected relevant study is analysed and then information are extracted. For this purpose, a data extraction form is generated and filled with the extracted information in order to be analyzed during the next step. More details are presented in Section \ref{sec:data_extraction}.

\item \textit{Data analysis}: Comprises the last step of conducting phase. A detailed and comprehensive analysis of the extracted information (performed in the previous step) is made in the form of different maps (i.e. plotting charts such as bubble charts, pie charts and graphs) and an analysis is made, with the aim to address each research question of our study. The details about this activity are in Section~\ref{sec:dataAnalysis}.

\end{enumerate}

%  \textcolor{SaraColor}{Sara: I suggest, if we used "we did ...or ... for (i) and (iv), it would be better to keep the text more harmonize and apply it for (ii), (iii), and (v) as well!!}
 
\textbf{ Documenting: } The last phase in the study process aims at (i) generating a detailed analysis of the extracted information in the previous phase and thorough explanations of the obtained results as presented in Section~\ref{sec:results}, (ii) the analysis of possible threats to validity see Section~\ref{sec:validity}.




==> 1st submission backup/validity.tex <==
\section{Threats to validity}
\label{sec:validity}

When conducting a systematic mapping study, there are usually some issues that might jeopardize the validity of the work. In this subsection, the method to mitigate the threats of validity is described, which follows the the guidelines of Wohlin et al. in \cite{wohlin2012experimentation}. 

%\begin{itemize}
\subsection{Construct validity} 

Construct validity in systematic mapping studies stresses the validity of the extracted data concerning the research questions. For this systematic mapping study, the guidelines in \cite{petersen2015guidelines} were followed. The selection of the primary studies represents the research questions in a confident way. Starting with the search string, it is well-formulated using the PICO method. Then, the most common digital libraries in software engineering were chosen to perform the automatic search, which gives more depth to the study as mentioned in Section \ref{sec:stringSource}. The publications collected by performing the search were reviewed with respect to their titles and abstracts. If a publication could not be judged for relevance based on its title and abstract, full-text skimming was performed to decide about its relevance in the research area. 

Furthermore, the studies were screened under rigorous inclusion and exclusion criteria. To be noted is that not using ``snowballing sampling'' might reduce the credibility of the study, but the big number of primary studies covers the desired scope. Considering all the above-mentioned, it is believed that no relevant studies were left out of the research.  
Moreover, the selection team members classified a certain number of common studies (170 out of 4808 studies have been randomly selected) to check the overall agreement, achieving 0.80 which shows almost perfect agreement.

\subsection{Internal validity} 
Internal validity represents those threats that seek to establish a causal relationship, where some conditions may influence the study. To mitigate this threat, a predefined protocol with an exact data extraction form was used. Regarding the data analysis, since descriptive statistics would be employed, the threats are minimal.  

Another threat is related to the classification schema for mapping. To mitigate,we partially based our classification of the primary studies on  initial  categorization, which is based on the discussions with experts from their respective fields and refined the categories further using few iterative meetings. Further, we systematically applied the keywording method to define the classification schemes. We believe that this process of classification would have refined our mapping to mitigate this threat.

\subsection{External validity} 

Threats to external validity define the extent of the generalizability of the outcomes of systematic mapping study. In this research, the most drastic threat related to external validity is not covering the whole scope of AI using communication technologies to provide safety. This threat is mitigated by a well-established search string and the automatic search. Having a good set of inclusion and exclusion criteria helped as well in the external validity of the study. However, since the T-A-K skimming was performed, due to abstracts with incomplete information, some relevant studies might have been wrongly excluded.
However, as it is known that abstracts do not always reveal the true content of papers, there is a risk that we might have excluded a paper with poor abstract but valid content.
%\textcolor{red}{Sara do we move your last para from Construct validity here?}

To further minimize the external threat, only the publications written in English (widely used language in qualitative scientific studies) were chosen and additionally only the peer-reviewed studies were accepted.
    
\subsection{Conclusion validity} 

Conclusion validity demonstrates that the study can be repeated in the future and yet have the same results. The relationship between the extracted and synthesized data and the outcomes of the study may influence the repetitiveness.

In order to mitigate this threat, all the steps leading to data analysis including search string, automatic search, selection criteria. are well-documented. They can be used by researchers to replicate the study. 
Furthermore, the data extraction form is well-documented, decreasing the biases of that process. The same reasoning is followed with the classification scheme as well, where the framework is well-defined and has the respective references. 


==> IntroRWRev1.tex <==
\section{Introduction}
\label{sec:introduction}

The advances in the \textit{Artificial Intelligence (AI)} field enabled different software systems to achieve higher levels of automation. This evolution moves towards a less dependence on human intervention for an intelligent system to make decisions~\cite{Alsamhi2019} %, Wollschlaeger2017}. 
This also brings the possibility to have systems that interacts with humans in different manners. However, autonomy and interaction mechanisms must be designed in a way to ensure safety of the whole ecosystem. Consequently, \textit{safety} becomes a key component of AI-based autonomous systems~\cite{Huang2020, Everitt2018}. 
%and specially for those systems where humans are directly interacting with. 
Some examples of these systems include in which autonomous agents (such as general purpose robots, autonomous vehicles and drones) are involved that can operate in a heterogeneous environment, intermixed with humans, and perform a broad spectrum of tasks~\cite{FordBookRobots, Guiochet2017, Bila2017, InamETFA18}. These smart autonomous agents are equipped with sensors and AI to operate in an automated or semi-automated fashion.

%and cooperate with each other and humans in a safe, autonomous, and reliable manner.  
%and destine to bring a new industrial revolution. 4th industrial revolution that is based on autonomous  and smart Cyber Physical Systems (CPSs) [2]
%AI is an integral part of 

The smart autonomous agents are part of a big and complex smart \textit{Cyber Physical System (CPS)} in which they cooperate with each other and humans in a safe, autonomous, and reliable manner. These agents are used in a vast set of application domains ranging from automotive industry, mining, agriculture, air space using unmanned aerial vehicles (UAV), healthcare, smart manufacturing, telecommunication, Internet-of-Things (IoT), and more~\cite{Bila2017, Guiochet2017, Kun-Hsing2018, Jha2019, Cayamcela2018, Islam2015}. AI algorithms usually require efficient hardware processing capabilities to train and execute, which is not always possible to do on the agent or device which usually have limited resources. Additionally, for safety-critical systems there are mostly real-time requirements to execute the algorithms. As an example, \textcolor{blue}{the processing of large amount of sensor data generated by autonomous vehicle must be made in real-time to avoid any accident. Thus, there is a need for AI-based safe operations and, at the same time, for powerful processing hardware.} %Thus, the need is of not only AI-based safe operations, but the access to 
%vast knowledge base and 
%powerful processing hardware is also essential. 

% These challenges make the \textit{communication} of the agents with each other and with powerful remote machines \textcolor{red}{Rafia: remote machines or remote algorithms or remote functions?} (could be at edge and/or cloud infrastructures) an integral part of the whole system. 

\textcolor{blue}{All these challenges make the \textit{communication} to remote agents and remote processing infrastructures (e.g. edge or cloud computing) an integral part of the whole system.}
Based on the system’s demands, the communication needs could be very different. Two main types of communication technologies that play a significant role in such systems are \textit{cellular}~\cite{Ullah2019} and \textit{non-cellular communications}~\cite{Saleh2018, Aceto2018}. These technologies must fulfil system requirements, otherwise, communication can introduce safety risks by not making the system able to respond in a precise and timely manner. 

%Because of these challenges,  these systems need communications between agents and processing units. are both safety and mission critical. Safety
%AI is present in diverse applications, ranging from autonomous vehicles to personal assistants. In these devices, access to a vast knowledge base and powerful processing hardware is essential. This is possible by communicating with remote servers, such as edge and cloud infrastructures. Therefore, communication technologies have an increasing importance in the automation process. 
%However, the communication technologies must fulfil established requirements, such as low latency and high throughput. Otherwise, communication can introduce safety risks by not making the system able to respond in a precise and timely manner. 

Notably, \textit{a strong correlation between AI, safety and communication} technologies exist and the progresses made in one field have a direct impact on the others~\cite{Fellan2018, Sharma2020}. Traditionally, these fields were treated separately, but more recently a plenty of work covers the integration of AI using communication technologies to implement safety in different application domains. This is reflected in the publications made in recent years, which supports the convergence of these areas~\cite{Ullah2019, Wollschlaeger2017, Fellan2018, sirohi2020convolutional}.%\textcolor{red}{Alberto please include new citation \cite{c} } 

% Traditionally, these fields were treated separately, but more recently a plenty of works that covers the integration of AI with communication or safety have been proposed [REF]. 
%%% TODO: briefly explain systematic mapping study, present differences and advantages.
%There were efforts to track the evolution in these field, such as ..., however none of them covered them at the same time....
\textbf{ Paper Contributions:} The main goal of this study is to identify, classify, analyze and to identify gaps in the state-of-the-art research publications that utilizes AI algorithm(s) using communication to achieve safety in diverse domains. The study exclusively focuses on software aspects. To target this goal, we construct a structured map of the available research literature by conducting a well-established methodology from Software Engineering research community called systematic  mapping~\cite{kitchenham2007guidelines, petersen2008systematic}.
Using the systematic mapping process, we searched and selected relevant studies, defined a classification framework, applied the classification on the shortlisted studies in relation to various AI algorithms and communication technologies used in different domains to implement safety, and analysed and discussed the obtained results. 
%We also identified the  gaps  in  the  current  research  on  the use  of  AI  algorithms  and  communication  technologies in  different  application  domains;  and  to investigate in  different  domains  which  of  the  non-cellular  communication  technologies  can  potentially  be  replaced  by  the cellular ones to implement AI-based safety. 

The main contributions of this study are: 
\begin{itemize}
    \item A systematic review of current methods or techniques of AI and communication technologies applied in different domains to implement safety and to identify gaps in it;
 \item An investigation on the potential possibility of replacement of non-cellular communication technologies by the cellular ones to implement AI-based safety;
 \item A discussion of the current challenges and emerging future research trends on the topic, from both industry and academia perspectives, and to identify the interest of the industry on the topic;
 \item  Investigate the maturity of the performed research and the research approaches in general by considering the research type;
 \item Observe trends in the community’s
research focus by considering the research contribution for finding the increased focus on developing new methods, models or tools;
\end{itemize}

To the best of our knowledge, this paper presents the first systematic investigation into the state of the art on safety using AI and communication technologies in different domains.

\textbf{Paper outline:} The paper is organized as follows: \autoref{sec:related_works} presents an overview of related studies that covers AI for safety or communication; \autoref{sec:study_method} describes each step of the process of the systematic mapping used in the current study; \autoref{sec:classscheme} presents the classification schemes developed
in this study; \autoref{sec:results} analyses the mapping results and provides the plots generated in the mapping process; \textcolor{blue}{\autoref{sec:validity} describes the threats to the validity of this work; and finally \autoref{sec:conclusions} concludes this systematic mapping.}

\section{Related Works}
\label{sec:related_works}

% mention surveys in the communication+AI, AI+safety fields

There are many efforts in the literature to provide a comprehensive study that cover AI to implement safety.
%or to communication. Regarding AI to implement safety, there are different works that make an extensive review in this field.
% \textcolor{red}{I think we mention clustering, image processing also here. Alberto can you find something on these? Image processing is a technique ... Clustering is heavily used in automotive domain \cite{}}
Neural networks (NNs) and more specifically, deep learning (DL) is a technique that is widely adopted in a variety of safety related problems. 
More recently, Huang et al. \cite{Huang2020} presents the growing interest to train safe DL models for critical applications (e.g. autonomous vehicles and autonomous surgery). The work of Huang explores a variety of strategies to ensure model safety, such as interpretability, verification and testing. Tran et al. \cite{Tran2020} presents an overview of verification methods to ensure the correctness of AI in safety systems. 
\textcolor{blue}{Fayyad et al. \cite{Fayyad2020} presents a study on the use of deep learning based algorithms for perception, localization, and mapping used in autonomous vehicle systems in short-range or local vehicle environments.}
Reinforcement learning (RL) is an AI technique that is getting more popular in safety applications. For instance, in \cite{Garcia2015} is made an overview of studies that employ a particular RL method that incorporates safety, named safe RL, which basically investigates techniques to ensure safe exploration. 
The combination of computer vision and safety also brought the interest of researchers to elaborate survey works as in \cite{Al-Kaff2018}. Clustering is also another AI algorithm that is getting attention, specially inside vehicular communication problems \cite{Cooper2017}.
There are also works that make analysis of safety in a more general context of AI. To exemplify, \cite{Leslie2019} presents a comprehensive study of AI ethics and safety, and compiles papers related to this field. While \cite{Everitt2018} reunites studies that discusses the safety of Artificial General Intelligence (AGI) algorithms. It covers studies that bring ideas of how AGI can be designed in a safe manner.

Additionally, there are literature review studies that analyse safety in different application domains. %Robotics is one such field, specially used in industries 4.0. 
\cite{Guiochet2017} discusses different solutions proposed by the scientific community to guarantee safety when interacting with robots. Similarly, \cite{Bila2017} presents strategies to avoid accidents in intelligent transportation systems (ITS) when dealing with unforeseen situations. AI in healthcare is a topic that is covered in the review article of \cite{Kun-Hsing2018}, which brings the usage of different AI methods and data infrastructure for medicine related problems. \textcolor{blue}{\cite{Pouyan2020} examines the perceived benefits and risks of AI medical devices with clinical decision support features from consumers' perspectives using an online survey based data from 307 individuals, and reveals that technological, ethical (trust factors), and regulatory concerns significantly contribute to the perceived risks of using AI applications in healthcare.} Agriculture is yet another area that has large application of AI, specially in problems related to automation as raised in the review study of \cite{Jha2019}. This work also highlights the use of communication technologies in the agricultural automation, specially in those solutions that involve Internet of Things (IoT).

Besides not having survey works covering safety in communication domain, there are plenty of studies that explore AI in communication domain. \cite{Tong2019}  covers different AI solutions employed together with vehicle-to-everything (V2X) communication to leverage traffic safety and efficiency. While in \cite{Alsamhi2019} AI is targeted for robot communication to enable complex decisions in a efficient way. In the cognitive radio field, which deals with dynamic reconfiguration of telecommunication networks, there are surveys studies that discusses the application of different AI algorithms as in \cite{Bkassiny2013} and \cite{Abbas2015}. Self-organizing network (SON) is a topic related to automation of telecommunication tasks that have derived literature review studies investigating the usage of different AI techniques \cite{Klaine2017}. The recent advent of 5G also brings survey that involves the employment of AI \cite{Cayamcela2018}. 
\textcolor{blue}{\cite{sirohi2020convolutional} study the use of convolutional neural networks (CNN) and their variants for object detection, localization, and classification in modern 5G enabled ITS. }
Moreover, there are also studies that narrows down to specific machine learning techniques, mainly deep learning \cite{Mao2018, Erpek2020} and reinforcement learning \cite{Luong2019}.

Another perspective explored by the studies is the relationship between the communication technologies and the different application domains. For example, there are survey studies that investigate different communication architectures and strategies used in the health care domain as presented in \cite{Islam2015, Saleh2018} and \cite{Aceto2018}. There are also studies that make a wider analysis of a particular communication technology in different domains. In \cite{Ullah2019}, the impact of 5G communication is addressed in intelligent transportation, drones and healthcare. With the rise of Industry 4.0, the communication in manufacturing field also has been investigated in \cite{Wollschlaeger2017} and \cite{Marcon2017}. Studies that cover communication for specific machines, such as automated grounded vehicles (UAV) and drones is presented in \cite{Fellan2018} and in \cite{Sharma2020}, respectively.

Our current study takes a different perspective from the previous works by providing analysis of studies that make use of AI and communication technology to provide safety in diverse domains. As shown in this section, these three key terms (AI, communication and safety) have been used separated or combined, but their simultaneous usage is neglected and is not covered so far to the best of our knowledge. As AI is getting more and more used in different fields, the safety of its application have a proportional importance. Likewise, communication and AI is even more related as both depends on each other either to provide an efficient communication or ensure the real-time execution through cloud computing. 

% Regarding studies that investigate AI to enhance communication technologies, there are a number of surveys that explores the usage of AI for telecommunication networks. Naturally, it can be found survey studies that involves the application of AI or ML for cognitive radio networks as in \cite{Bkassiny2013} and \cite{Abbas2015}, and self-organizing networks as in \cite{Klaine2017}. The recent advent of 5G also brings survey that involves the employment of AI \cite{Cayamcela2018}. Moreover, there are also studies that narrows down to specific machine learning techniques, mainly deep learning \cite{Mao2018, Erpek2020} and reinforcement learning \cite{Luong2019}.

%% AI + Safety works
% On the Safety of Machine Learning: Cyber-Physical Systems, Decision Sciences, and Data Products
% https://www.liebertpub.com/doi/abs/10.1089/big.2016.0051
% MachineLearningSafety:An Overview
% https://www.researchgate.net/profile/Jose_Faria12/publication/320567319_Machine_Learning_Safety_An_Overview/links/59f37efda6fdcc075ec34986/Machine-Learning-Safety-An-Overview.pdf
% A Comprehensive Survey on Safe Reinforcement Learning
% https://pdfs.semanticscholar.org/c0f2/c4104ef6e36bb67022001179887e6600d24d.pdf
% AGI Safety Literature Review
% https://arxiv.org/pdf/1805.01109.pdf

%% AI + Safety applications
% Safety-critical advanced robots: A survey
% https://www.sciencedirect.com/science/article/abs/pii/S0921889016300768
% Vehicles of the Future: A Survey of Research on Safety Issues
% https://ieeexplore.ieee.org/abstract/document/7559813

%% AI + Communications
% Artificial Intelligence-Based Techniques for Emerging Robotics Communication: A Survey and Future Perspectives
% https://arxiv.org/abs/1804.09671
%  A Survey on Machine-Learning Techniques in Cognitive Radios 
% https://ieeexplore.ieee.org/abstract/document/6336689
% Recent advances on artificial intelligence and learning techniques in cognitive radio networks
% https://link.springer.com/article/10.1186/s13638-015-0381-7
% A Survey of Machine Learning Techniques Applied to Self-Organizing Cellular Networks
% https://ieeexplore.ieee.org/abstract/document/7982603/authors#authors
% https://ieeexplore.ieee.org/abstract/document/8543584
% Artificial Intelligence in 5G Technology: A Survey
% https://ieeexplore.ieee.org/document/8539642

% Applications of Deep Reinforcement Learning in Communications and Networking: A Survey
% https://ieeexplore.ieee.org/abstract/document/8714026
% Deep Learning for Wireless Communications
% https://link.springer.com/chapter/10.1007/978-3-030-31764-5_9
% Deep Learning for Intelligent Wireless Networks: A Comprehensive Survey 
% https://ieeexplore.ieee.org/abstract/document/8382166
% A survey of deep learning-based network anomaly detection
% https://link.springer.com/article/10.1007/s10586-017-1117-8
% Towards the Deployment of Machine Learning Solutions in Network Traffic Classification: A Systematic Survey
 
% https://ieeexplore.ieee.org/abstract/document/8539642/authors#authors

% A survey of recent advances in fuzzy logic in telecommunications networks and new challenges
% https://ieeexplore.ieee.org/abstract/document/705512
% Resource Allocation for Network Slicing in 5G Telecommunication Networks: A Survey of Principles and Models
% https://ieeexplore.ieee.org/abstract/document/8770537

